Automated Scientific Discovery: From Equation Discovery to Autonomous Discovery Systems

The paper surveys automated scientific discovery, from equation discovery and symbolic regression to autonomous discovery systems and agents. It discusses the individual approaches from a "big picture" perspective and in context, but also discusses open issues and recent topics like the various roles of deep neural networks in this area, aiding in the discovery of human-interpretable knowledge. Further, we will present closed-loop scientific discovery systems, starting with the pioneering work on the Adam system up to current efforts in fields from material science to astronomy. Finally, we will elaborate on autonomy from a machine learning perspective, but also in analogy to the autonomy levels in autonomous driving. The maximal level, level five, is defined to require no human intervention at all in the production of scientific knowledge. Achieving this is one step towards solving the Nobel Turing Grand Challenge to develop AI Scientists: AI systems capable of making Nobel-quality scientific discoveries highly autonomously at a level comparable, and possibly superior, to the best human scientists by 2050.

==> tables/systems.tex <==


\begin{table}[h]
    \centering
    \caption{Ten prominent examples of efforts for closed-loop scientific discovery from seven different countries and across six different disciplines.}
    \begin{tabular}{|l|l|p{4.5cm}|l|}
        \hline
        \textbf{Discipline} & \textbf{Name} & \textbf{Link} & \textbf{Country} \\
        \hline
        Drug Discovery & Eve & \href{https://www.chalmers.se/en/departments/bio/news/Pages/Chalmers-Robot-Scientist-ready-for-drug-discovery.aspx}{Chalmers Robot Scientist} & Sweden \\
        \hline
        Drug Discovery & Recursion & \href{https://www.recursion.com/}{Recursion} & US \\
        \hline
        Drug Discovery & Lilly Life Sciences Studio lab & \href{https://investor.lilly.com/news-releases/news-release-details/eli-lilly-and-company-collaboration-strateos-inc-launch-remote}{Lilly Life Sciences} & US \\
        \hline
        Chemistry & roboRXN at IBM & \href{https://research.ibm.com/science/ibm-roborxn}{IBM roboRXN} & Switzerland \\
        \hline
        Chemistry & AI-Chemist & \href{https://academic.oup.com/nsr/article/9/10/nwac190/6694008}{AI-Chemist} & China \\
        \hline
        Materials/Biology & Argonne Autonomous Discovery & \href{https://www.anl.gov/autonomous-discovery/developing-a-selfdriving-laboratory-prototype}{Argonne Autonomous Discovery} & US \\
        \hline
        Materials & Robot Chemist & \href{https://www.liverpool.ac.uk/leverhulme-research-centre/news/articles/feature-will-we-ever-have-a-robo-chemist/}{Robot Chemist} & UK \\
        \hline
        Materials & Acceleration Consortium & \href{https://acceleration.utoronto.ca/}{Acceleration Consortium} & Canada \\
        \hline
        Bioprocessing & KIWI-lab & \href{https://kiwi-biolab.de}{KIWI-lab} & Germany \\
        \hline
        Astronomy & Automated Planet Finder (APF) & \href{https://www.ucolick.org/public/telescopes/apf.html}{Automated Planet Finder (APF)} & US \\
        \hline
    \end{tabular}
    \label{tab:automation_list}
\end{table}


